Incremental Parsing with Minimal Features Using Bi-Directional LSTM

Recently, neural network approaches for parsing have largely automated the combination of individual features, but still rely on (often a larger number of) atomic features created from human linguistic intuition, and potentially omitting important global context. To further reduce feature engineering to the bare minimum, we use bi-directional LSTM sentence representations to model a parser state with only three sentence positions, which automatically identifies important aspects of the entire sentence. This model achieves state-of-the-art results among greedy dependency parsers for English. We also introduce a novel transition system for constituency parsing which does not require binarization, and together with the above architecture, achieves state-of-the-art results among greedy parsers for both English and Chinese.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
#figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	#@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "15 15 15 15" main.pdf

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile


==> sr.tex <==
%\subsection{Extended Shift-Reduce}
\label{sec:esr}
One major challenge in constituency parsing is unary rules.
Unlike dependency parsing
where shift-reduce always finishes in $2n-1$ steps,
existing incremental constituency parsers~\cite{zhu+:2013,wang+xue:2014}
reach the goal state (full parse tree) in different steps due to different number of unary rules.
So we propose a new, synchronized, ``odd-even'' system to reach the goal in the same $4n-2$ steps.
%% Our shift-reduce parser performs a sequence of steps
%% to parse the input sentence in a left-to-right manner, 
A {\it state} is notated $p = \langle S, Q \rangle$,
where $S$ is a stack of trees $..., s_1, s_0$, and $Q$ is 
a queue of word-tag pairs. 
At even steps (when step index is even) we can choose one of the three standard actions %(see Figure~\ref{fig:esr}): 
\begin{itemize}
\item \shift: %if $s_0$ has a star mark, $s^*_0$, or $S$ is empty $\epsilon$, 
shift the head of $Q$, a word-tag pair ($t, w$), onto $S$ 
as a singleton tree $t(w)$; % without marking;
\item \lreducex: %if the top two trees on stack both have star marks ($s^*_1$ and $s^*_0$), 
combine the top two trees on the stack and replace them with a new tree $x(s_1, s_0)$, $x$ being the root nonterminal, headed on $s_0$;
\item \rreducex: similar to \lreducex but headed on $s_1$;
\end{itemize}
and at odd steps we can choose two new actions:
\begin{itemize}
%if both $s_1$ and $s_0$ have star marks, $s^*_1$ and $s^*_0$,
%combine them and replace them with a new tree $x(s_1, s_0)$ headed on $s_1$;
\item \unaryx: %if $s_0$ doesn't have a star mark, 
replace $s_0$ with a new tree $x(s_0)$ with $x$ being the root nonterminal;
\item \stay: no action.
%if $s_0$ doesn't have a star mark, mark it as $s^*_0$.
\end{itemize}



\begin{figure}
\tabcolsep=0.05cm
\begin{tabular}{cl}
input & $(t_1, w_1)$ ... $(t_{n}, w_{n})$ \\
 & \\
axiom & $0: \langle \epsilon, (t_1, w_1)$ ... $(t_{n}, w_{n}) \rangle : 0$ \\
 & \\
\shift & $\cfrac{l : \langle S, (t,w) | Q \rangle : c}{l{\text +}1 : \langle S|t(w), Q \rangle : c {\text +} c_{\shift}}$  
$l$ is even\\
%{\small $S$ = $\epsilon$ or $S'|s_0$} \\
 & \\
\lreducex & $\cfrac{l : \langle S | s_1 | s_0, Q \rangle : c}{l{\text +}1 : \langle S|x(s_1,s_0), Q \rangle: c {\text +} c_{\lreducex} }$ $l$ is even\\
  & \\
%% \rreducex & $\cfrac{l : \langle S | s_1 | s_0, Q \rangle : c}{l{\text +}1 : \langle S|x(s_1,s_0), Q \rangle: c {\text +} c_{\rreducex} }$ \\
%%  & \\
\unaryx & $\cfrac{l : \langle S | s_0, Q \rangle : c}{l{\text +}1 : \langle  S|x(s_0), Q \rangle: c {\text +} c_{\unaryx} }$ $l$ is odd\\
 & \\
\stay & $\cfrac{l : \langle S | s_0, Q \rangle : c}{l{\text +}1 : \langle  S|s_0, Q \rangle: c {\text +} c_{\stay} }$ $l$ is odd\\
 & \\
goal & $2(2n-1)$ : $\langle s_0, \epsilon \rangle$ : $c$ \\ 
\end{tabular}
\caption{Shift-reduce system, omitting \rreducex. $c$ is the model score, 
and $c_\shift$, $c_\lreducex$, etc.~are the action scores. \label{fig:esr}}
%\vspace{-0.2cm}
\end{figure}

Figure~\ref{fig:esr} shows the deductive system. 
Note that we alternate between standard shift-reduce actions in even steps
and unary actions (\unaryx or \stay) in odd steps,
and the first action must be \shift, followed by 
a \unaryx or \stay, and followed by another \shift.
%% all actions are fired on conditions, and 
%% all reduce actions (\lreducex or \rreducex) are binary operations. 
%% For example,
%% starting with the axiom, we can only apply an \shift action.
%% Then, we apply an \unaryx or \stay action. In the next step,
%% we apply an \shift action, followed by an \unaryx or \stay action.
%% If we have $s^*_0$ and $s^*_1$, we can fire reduce actions. 
Continuing this procedure, %we find following good properties.
we can always achieve the goal in  $2(2n-1)$ steps.
%% Second, we actually fire \shift, \lreduce and \rreduce 
%% actions in odd steps, \unaryx and \stay in even steps, 
%% thus, we don't apply two consecutive unary (\unaryx or \stay) actions. 
%and in a same beam different states have a same number of unary actions.


In practice, we have larger than two-way rules and multi-level unary rules,
so we binarize them and collapse multi-level unary rules into one level,
for example,

\scalebox{0.9}{
\begin{tabular}{ccc}
\tikzset{level distance=0.75cm} \Tree [.NP [.S [.VP [.V ] [.NP ] [.PP ] ] ] ] 
& \tikzset{edge from parent/.style={draw, edge from parent path={(\tikzparentnode) (\tikzchildnode)}}} 
  \Tree [.{} [. $\Longrightarrow$ ] ] 
& \tikzset{level distance=0.75cm} \Tree [.NP+S [.VP [.VP$'$ [.V ] [.NP ] ] [.PP ] ] ] \\
\end{tabular}
}
\smallskip
% \begin{enumerate}
% \item[] (IP (NP (NR $w$))) $\goesto$ (IP+NP (NR $w$)). 
% \end{enumerate}

%\subsection{Features}

Following \namecite{huang+sagae:2010}, 
we represent {\bf feature templates}
as functions 
$\mathbf{f}(\cdot,\cdot)$ on stack $S$ and
queue $Q$.
Table~\ref{tab:feats} shows the 43 feature templates we use in this paper,
all adopted from \namecite{zhu+:2013}.
They are combinations of the 
$32$ {\bf atomic features} $\mathbf{\tilde{f}}(S, Q)$
%defined as the smallest set of features
(e.g. $s_0.\ft$ and $s_0.\fc$  denote the head tag and syntactic category
of tree $s_0$, resp.,
and $s_0.\flc.\fw$ is the head word of its leftmost child).

 
\begin{table*}
\small
\centering
\tabcolsep=0.1cm
\scalebox{0.9}{
\begin{tabular}{ccccccc}
\hline
  \multicolumn{7}{c}{feature templates $\mathbf{f}(S, Q)$} \\
\hline
%\multicolumn{7}{c}{unigrams}  \\
unigrams & $s_0.\ft \circ s_0.\fc$ & $s_0.\fw \circ s_0.\fc $ 
         & $s_1.\ft \circ s_1.\fc$ &$s_1.\fw \circ s_1.\fc$ & $s_2.\ft \circ s_2.\fc$ & $s_2.\fw \circ s_2.\fc$\\
         & $s_3.\ft \circ s_3.\fc$ & $q_0.\fw \circ q_0.\ft $ & $q_1.\fw \circ q_1.\ft$ 
         & $q_2.\fw \circ q_2.\ft$ & $q_3.\fw \circ q_3.\ft$ & $s_0.\flc.\fw \circ s_0.\flc.\fc$\\
         & $s_0.\frc.\fw \circ s_0.\frc.\fc$ & $s_0.\fu.\fw \circ s_0.\fu.\fc$ 
         & $s_1.\flc.\fw \circ s_1.\flc.\fc$ & $s_1.\frc.\fw \circ s_1.\frc.\fc$ & $s_1.\fu.\fw \circ s_1.\fu.\fc$ \\
\hline
%\multicolumn{6}{c}{bigrams}  \\ 
bigrams & $s_0.\fw \circ s_1.\fw$ & $s_0.\fw \circ s_1.\fc $ & $s_0.\fc \circ s_1.\fw$ 
        & $s_0.\fc \circ s_1.\fc$ & $s_0.\fw \circ q_0.\fw$ & $s_0.\fw \circ q_0.\ft$\\
        & $s_0.\fc \circ q_0.\fw$ & $s_0.\fc \circ q_0.\ft $ & $q_0.\fw \circ q_1.\fw$ 
        &$q_0.\fw \circ q_1.\ft$ & $q_0.\ft \circ q_1.\fw$ & $q_0.\ft \circ q_1.\ft$\\
        & $s_1.\fw \circ q_0.\fw$ & $s_1.\fw \circ q_0.\ft$ & $s_1.\fc \circ q_0.\fw$ & $s_1.\fc \circ q_0.\ft$ &  &  \\
        & \multicolumn{2}{c}{$s_0.\fc \circ s_0.\flc.\fc \circ s_0.\frc.\fc \circ s_1.\fc $} 
        & \multicolumn{2}{c}{$s_0.\fc \circ s_0.\flc.\fc \circ s_0.\frc.\fc \circ s_1.\fc $} &  & \\
\hline
%\multicolumn{6}{c}{trigrams}  \\
trigrams & \multicolumn{2}{c}{$s_0.\fc \circ s_1.\fc \circ s_2.\fc$} 
         & \multicolumn{2}{c}{$s_0.\fw \circ s_1.\fc \circ s_2.\fc$} 
         & \multicolumn{2}{c}{$s_0.\fc \circ s_1.\fw \circ q_0.\ft$} \\
         & \multicolumn{2}{c}{$s_0.\fc \circ s_1.\fc \circ s_2.\fw$} 
         & \multicolumn{2}{c}{$s_0.\fc \circ s_1.\fc \circ q_0.\ft$} 
         & \multicolumn{2}{c}{$s_0.\fw \circ s_1.\fc \circ q_0.\ft$} \\
         & \multicolumn{2}{c}{$s_0.\fc \circ s_1.\fw \circ q_0.\ft$} 
         & \multicolumn{2}{c}{$s_0.\fc \circ s_1.\fc \circ q_0.\fw$} & &  \\
\hline
\end{tabular}
}
%\vspace{-0.1cm}
\caption{All feature templates ($43$ templates based on $32$ atomic features), taken from \namecite{zhu+:2013}.
$s_i.\fc$, $s_i.\fw$ and $s_i.\ft$ denote
the syntactic label, the head word, and the head tag of $s_i$.
$s_i.\flc.\fw$ means the head word of the left child of $s_i$.
$s_i.\fu.\fw$ means the head word of the unary root $s_i$.
$q_i.\fw$ and $q_i.\ft$ denote the word and the tag of $q_i$.
\label{tab:feats}}
%\vspace{-0.3cm}
\end{table*}



